Knowledge-Prompted Estimator: A Novel Approach to Explainable Machine Translation Assessment

Cross-lingual Machine Translation (MT) quality estimation plays a crucial role in evaluating translation performance. GEMBA, the first MT quality assessment metric based on Large Language Models (LLMs), employs one-step prompting to achieve state-of-the-art (SOTA) in system-level MT quality estimation; however, it lacks segment-level analysis. In contrast, Chain-of-Thought (CoT) prompting outperforms one-step prompting by offering improved reasoning and explainability. In this paper, we introduce Knowledge-Prompted Estimator (KPE), a CoT prompting method that combines three one-step prompting techniques, including perplexity, token-level similarity, and sentence-level similarity. This method attains enhanced performance for segment-level estimation compared with previous deep learning models and one-step prompting approaches. Furthermore, supplementary experiments on word-level visualized alignment demonstrate that our KPE method significantly improves token alignment compared with earlier models and provides better interpretability for MT quality estimation. Code will be released upon publication.

==> 030background.tex <==

\subsection{Non-Autoregressive Translation}


==> 060results.tex <==








==> tables/case_study.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabularx}{\linewidth}{|X|}
    \hline
        \multicolumn{1}{|c|}{\textbf{Case 1}}\\
        \hline
        \textbf{Source} \\
        However, carriages are also popular for \textcolor{teal}{hen parties}, he commented.\\
        \hline
        \textbf{Target} \\
        Kutschen sind aber auch für \textcolor{brown}{Jungesellinnenabschiede} beliebt, meint er.\\
        \hline
        \textbf{Terminology Constraints} \\
        \textcolor{teal}{hen parties} $\rightarrow$ \textcolor{brown}{Jungesellinnenabschiede} \\
        \hline
        \hline
        \multicolumn{1}{|c|}{{LevT}}\\
        \hline
        \textbf{Unconstrained translation}\\
        Kutschen sind aber auch für \textit{\textcolor{red}{Hühnerfeiern}} beliebt, kommentierte er.
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \
        $\Rightarrow$ \textit{{wrong term}}\\
        \hline
        \textbf{Soft constrained translation} \\
        Allerdings sind auch für \textit{\textcolor{red}{Hinnenabschiebeliebt}}, kommentierte er.
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
        $\Rightarrow$  \textit{{wrong term}}\\
        \hline
        \textbf{Hard constrained translation}\\
        Aber Auch für \textit{\textcolor{brown}{Jungesellinnenabschiede}} sind beliebt, sagte er.
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
        $\Rightarrow$ \textit{{incomplete sentence}} \\
        \hline
        \hline
        \multicolumn{1}{|c|}{{LevT + ACT}}\\
        \hline
         \textbf{Unconstrained translation}\\
        Wagen sind aber auch für \textit{\textcolor{red}{Hühnerpartys}} beliebt, kommentierte er.
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \
        $\Rightarrow$ \textit{{wrong term}}\\
        \hline
        \textbf{Soft constrained translation} \\
        Kutschen sind aber auch für \textit{\textcolor{brown}{Jungesellinnenabschiede}} beliebt, sagte er.\\
        \hline
        \textbf{Hard constrained translation}\\
        Kutschen sind aber auch für \textit{\textcolor{brown}{Jungesellinnenabschiede}} beliebt, sagte er. \\
        \hline
        \hline
        \hline
        \multicolumn{1}{|c|}{\textbf{Case 2}}\\
        \hline
        \textbf{Source} \\
        The media also reported that several people \textcolor{teal}{injured}.\\
        \hline
        \textbf{Target} \\
        Medien berichteten außerdem von mehreren \textcolor{brown}{Verletzten}.\\
        \hline
        \textbf{Terminology Constraints} \\
        \textcolor{teal}{injured} $\rightarrow$ \textcolor{brown}{Verletzten} \\
        \hline
        \hline
        \multicolumn{1}{|c|}{{LevT}}\\
        \hline
        \textbf{Unconstrained translation}\\
        Die Medien berichteten auch, dass mehrere Menschen \textit{\textcolor{red}{verletzt}} wurden.
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
        $\Rightarrow$ \textit{{wrong term}}\\
        \hline
        \textbf{Soft constrained translation} \\
        Die Medien berichteten auch, dass mehrere \textit{\textcolor{red}{Verletzte}} wurden.\ \ 
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \
        $\Rightarrow$  \textit{{wrong term}}\\
        \hline
        \textbf{Hard constrained translation}\\
        Die Medien berichteten auch, dass mehrere \textit{\textcolor{red}{Verletzte}} wurden. 
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
        $\Rightarrow$ \textit{{wrong term}} \\
        \hline
        \hline
        \multicolumn{1}{|c|}{{LevT + ACT}}\\
        \hline
        \textbf{Unconstrained translation}\\
        Die Medien berichteten auch, dass mehrere Menschen \textit{\textcolor{red}{verletzt}} wurden.
        \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  
        $\Rightarrow$ \textit{{wrong term}}\\
        \hline
        \textbf{Soft constrained translation} \\
        Die Medien berichteten auch, dass mehrere \textit{\textcolor{brown}{Verletzten}}.\\
        \hline
        \textbf{Hard constrained translation}\\
        Die Medien berichteten auch, dass mehrere \textit{\textcolor{brown}{Verletzten}}.\\
    \hline
    \end{tabularx}
    \caption{Case study of \levt and \levt with ACT.
    \textcolor{brown}{Text in brown} denotes the constraint word, \textcolor{red}{text in red} denotes the translation error of constraints, and $\Rightarrow$ denotes analysis of the translation errors.
    }
    \label{tab:casestudy}
\end{table}

==> tables/datasets.tex <==

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lccc}
    \toprule
    \textbf{Dataset} & \multirow{2}{*}{\textbf{\# Sent.}} & \textbf{Avg. Len.} & \textbf{Avg. Con.} \\
    (test set) &  & \textbf{of Con.} & \textbf{Freq.} \\
    \midrule
    WMT14-WIKT & 454 & 1.15 & 25,724.73 \\
    % WMT16-WIKT & 270 & 1.11 & 2214.85 \\
    WMT17-IATE & 414 & 1.09 & 3,685.42 \\
    WMT17-WIKT & 728 & 1.22 & 26,252.70 \\
    \hdashline
    OPUS-EMEA  & 2,996 & 1.95 & 2,187.63 \\
    OPUS-JRC  & 2,984 & 1.99 & 3,725.71 \\
    % \hdashline
    % WMT14-Full & 3,003 & - & - \\
    % WMT16-Full & 1,999 & - & - \\
    \bottomrule
    \end{tabular}
    \caption{Statistics of the test sets with target-side lexical constraints.
    ``\textbf{Avg. Len. of Con.}'' denotes the average number of words in a constraint.
    ``\textbf{Avg. Con. Freq.}'' is the average frequency of lexical constraints calculated with the training vocabularies of corresponding language.
    % All test sets are En$\rightarrow$De tasks except for WMT16-WIKT (Ro$\rightarrow$En).
    % Note that WMT14-WIKT are subsets of WMT14,  containing extracted lexical constraints.
    }
\label{tab:datasets}
\end{table}

==> tables/domain_results.tex <==

\begin{table}
    \centering
    \small
    \begin{tabular}{lccccc}
        \toprule
        \multirow{2}*{\textbf{Model}} & \multicolumn{2}{c}{\textbf{OPUS-EMEA}} & \multicolumn{2}{c}{\textbf{OPUS-JRC}} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        & \multicolumn{1}{c}{Term\%} & BLEU & \multicolumn{1}{c}{Term\%} & BLEU \\ 
        \midrule
        % Transformer$^\dagger$ & ? & ? & ? & ? \\
        % \hdashline
        LevT$^\dagger$ & 52.40 & 27.90 & \textbf{55.39} & 30.24 \\
        \ \ + ACT$^\dagger$ & \textbf{53.41} & \textbf{28.30} & 55.35 & \textbf{31.01} \\
        \hdashline
        \levt w/ \emph{soft} & 83.37  & 30.35 & 84.32 & 32.53 \\
        \ \ + ACT & \textbf{92.09} & \textbf{32.02} & \textbf{91.94} & \textbf{33.70} \\
        \hdashline
        \levt w/ \emph{hard} & 100.00 & 30.77 & 100.00 & 30.08 \\
        \ \ + ACT & 100.00 & \textbf{32.30} & 100.00 & \textbf{34.09} \\
        \bottomrule
    \end{tabular}
    \caption{Experiments on test sets from OPUS, which is outside the training set (WMT14 En$\rightarrow$De).
    Results shows ACT brings larger performance for lower-frequency lexical constraints within these datasets.}
    \label{tab:domain-result}
\end{table}


==> tables/freq_ablation.tex <==

\begin{table*}
    \centering
    \small
    \begin{tabular}{lcccccccccccc}
    \toprule
        \multirow{2}*{\textbf{Model}} & \multicolumn{4}{c}{\textbf{WMT14-WIKT}} & \multicolumn{4}{c}{\textbf{WMT17-IATE}} & \multicolumn{4}{c}{\textbf{WMT17-WIKT}} \\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    \cmidrule(lr){10-13}
        & \textsc{All} & \textsc{High} & \textsc{Med.} & \textsc{Low} & 
        \textsc{All} & \textsc{High} & \textsc{Med.} & \textsc{Low} &
        \textsc{All} & \textsc{High} & \textsc{Med.} & \textsc{Low}\\ 
     \midrule
        LevT$^\dagger$ & 29.95 & 30.46 & \textbf{28.03} & 31.49 & \textbf{29.80} &  \textbf{30.08} & \textbf{29.72} & \textbf{29.45} & \textbf{30.75} & \textbf{30.96} & 29.09 & 32.16 \\
        \ \  + ACT$^\dagger$ & \textbf{30.35} & \textbf{30.68} & 28.00 & \textbf{32.54} & 29.57 & 29.63 & 29.57 & 29.20 & 30.63 & 30.35 & \textbf{29.11} & \textbf{32.46} \\
        \hdashline
        \levt w/ \emph{soft}  & 30.38 & 30.37 & 28.50 & 32.19 & 30.11 &  29.25 & 30.67 & 30.04 & 30.92 &  30.70 & \textbf{29.58} & 32.23 \\
        \ \  + ACT  & \textbf{31.08} &  \textbf{30.48} & \textbf{29.18} & {\textbf{33.85}} & \textbf{30.56} &  \textbf{29.93} & \textbf{31.05} & \textbf{30.36} & \textbf{31.06} & \textbf{30.72} & 29.53 & \textbf{32.73} \\
         \hdashline
        \levt w/ \emph{hard}  & 30.49 &  \textbf{30.50} & 28.67 & 31.99 & 30.31 & 29.46 & 30.66 & 30.37 & 30.65 &  30.28 & 29.44 & 32.00 \\
        \ \  + ACT  & \textbf{31.11} & 30.23 & \textbf{29.32} & {\textbf{33.85}} & \textbf{30.68} &  \textbf{29.97} & \textbf{31.18} & \textbf{30.67} & \textbf{31.18} & \textbf{30.58} & \textbf{29.71} & \textbf{32.90} \\
     \bottomrule
    \end{tabular}
    \caption{
    Ablation results of terminology-constrained En$\rightarrow$De translation tasks w.r.t. word frequency of terms.}
    \label{tab:main-result-freq}
\end{table*}

==> tables/front.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{|l|}
    \hline
        \textbf{Source} \\
        $
        \underbrace{\mathrm{Travellers}}_\mathrm{1.8K} \underbrace{\mathrm{\textcolor{teal}{screamed}}}_\mathrm{\textcolor{teal}{24}} \underbrace{\mathrm{and}}_\mathrm{2.8M} \underbrace{\mathrm{children}}_\mathrm{30.0K} \underbrace{\mathrm{cried}}_\mathrm{122}.
        $ \\
        \hline
        \textbf{Target} \\
        $
        \underbrace{\mathrm{Reisende}}_\mathrm{944}
        \underbrace{\mathrm{h"atten}}_\mathrm{9.9K}
        \underbrace{\mathrm{\textcolor{brown}{geschrien}}}_\mathrm{\textcolor{brown}{13}}
        \underbrace{\mathrm{und}}_\mathrm{2.6M}
        \underbrace{\mathrm{Kinder}}_\mathrm{20.1K}
        \underbrace{\mathrm{geweint}}_\mathrm{13}.
        $ \\
        % Reisende hätten \textcolor{brown}{geschrien} und Kinder geweint.\\
        \hline
        \textbf{Terminology Constraints} \\
        \textcolor{teal}{scream} $\rightarrow$ \textcolor{brown}{geschrien}\\
        % (\textit{\textcolor{brown}{frequency}: 13})\\
        \hline
        \hline
        \textbf{Unconstrained translation}\\
        Reisende \textit{\textcolor{red}{schrien}} und Kinder rieen. \ \ \ \ \ \ $\Rightarrow$ \textit{{wrong term}}\\
        \hline
        \textbf{Soft constrained translation} \\
        Reisende \textit{\textcolor{red}{rien}}. \ \ $\Rightarrow$ \textit{{incomplete sentence}} \& \textit{{wrong term}}\\
        \hline
        \textbf{Hard constrained translation}\\
        Reisende \textit{\textcolor{brown}{geschrien}}. \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $\Rightarrow$ \textit{{incomplete sentence}} \\
    \hline
    \end{tabular}
    \caption{Translation examples of a lexically constrained non-autoregressive translation (NAT) model \cite{NEURIPS2019_675f9820} under a low-frequency word as constraint.
    The underbraced word frequencies (uncased) are calculated from the vast WMT14 English-German translation (En-De) datasets \cite{NIPS2017_3f5ee243}.
    % ``\textcolor{brown}{geschrien}'' has the frequency of only 13 in a vast corpus in German from WMT14 English$\rightarrow$German translation (En$\rightarrow$De) task \cite{NIPS2017_3f5ee243}.
    % \textcolor{red}{Text in red} means translation error of constraints, and $\Rightarrow$ denotes analysis of the translation errors.
    }
    \label{tab:front}
\end{table}

==> tables/main_results.tex <==


\begin{table*}[t]
    \small
    \centering
    \begin{tabular}{l||cc|cc|cc|c}
        \hline
        \multirow{2}*{\textbf{Models}} & \multicolumn{2}{c|}{\textbf{WMT17-IATE}} & \multicolumn{2}{c|}{\textbf{WMT17-WIKT}} & 
        \multicolumn{2}{c|}{\textbf{WMT14-WIKT}} & \textbf{Latency} \\
        & Term\% & BLEU & Term\% & BLEU & Term\% & BLEU & (ms)\\ 
        \hline
        \multicolumn{8}{l}{\textit{Reported results in previous work}}\\
        \hline
        Transformer \cite{NIPS2017_3f5ee243}$^\dagger$ & 79.65 & 29.58 & 79.75 & 30.80 & 76.77 & 31.75 & 244.5   \\
        DBA \cite{post-vilar-2018-fast} & 82.00 & 25.30 & 99.50 & 25.80 & - & - & 434.4  \\
        Train-by-rep \cite{dinu-etal-2019-training} & 94.50 & 26.00 & 93.40 & 26.30& - & - & -  \\
        \hdashline
        \levt \cite{NEURIPS2019_675f9820}$^\dagger$ & 80.31 & 28.97 & 81.11 & 30.24 & 80.23 & 29.86 & 92.0  \\
        \ \ w/ \emph{soft constraint} \cite{susanto-etal-2020-lexically} & 93.81 & 29.73 & 93.44 & 30.82 & 94.43 & 29.93 & -  \\
        \ \ w/ \emph{hard constraint} \cite{susanto-etal-2020-lexically} & \textbf{100.00} & \textbf{30.13} & \textbf{100.00} & \textbf{31.20} & \textbf{100.00} & \textbf{30.49} & -  \\
        \editor \cite{10.1162/tacl_a_00368}$^\dagger$ & 83.00 & 27.90 & 83.50 & 28.80 & - & - & 121.7  \\
        \ \ w/ \emph{soft constraint} & 97.10 & 28.80 & 96.80 & 29.30 & - & - & -  \\ 
        \ \ w/ \emph{hard constraint} & 100.00 & 28.90 & 99.80 & 29.30 & - & - & 134.1  \\
        \hline 
        \multicolumn{8}{l}{\textit{Our implementation}}\\
        \hline
        LevT$^\dagger$ & 78.32 & \textbf{29.80} & 80.20 & 30.75 & \textbf{79.53} & 29.95 & \textbf{71.9}  \\
        \ \ + constrained training (CT)$^\dagger$ & 78.76 & 29.46 & \textbf{80.77} & \textbf{30.82} & 79.13 & {30.24} & 78.6  \\
        \ \ + aligned constrained training (ACT)$^\dagger$ & \textbf{79.43} & 29.57 & 80.20 & 30.63 & 77.17 & {\textbf{30.35}} & 77.0  \\
        \hdashline
        \levt w/ \emph{soft constraint} & 94.25  & 30.11 & 93.78 & 30.92 & 94.88 & 30.38 & 79.5  \\
        \ \ + constrained training (CT) & 96.24 & 30.19 & 96.61 & 30.96 & 97.44 & {31.01} & \textbf{75.4}  \\
        \ \ + aligned constrained training (ACT) & \textbf{96.90} & {\textbf{30.56}} & \textbf{97.62} & \textbf{31.06} & \textbf{98.82} & {\textbf{31.08}} & 76.3  \\
        \hdashline
        \levt w/ \emph{hard constraint} & 100.00 & 30.31 & 100.00 & 30.65 & 100.00 & 30.49 & 82.7  \\
        \ \ + constrained training (CT) & 100.00 & 30.31 & 100.00 & 30.99 & 100.00 & 31.01 & 78.1  \\
        \ \ + aligned constrained training (ACT) & 100.00 & \textbf{30.68} & 100.00 & \textbf{31.18} & 100.00 & \textbf{31.11} & \textbf{77.0}  \\
        \hline
    \end{tabular}
    \caption{Translation results with lexical constraints.
    \textbf{Term\%} is the constraint term usage rate.
    Method$^\dagger$ translates \textit{without} lexical constraints in input. 
    % {Underlined result} indicates the improvement over \levt is significant ($p < 0.05$).
    }
    \label{tab:main-result}
\end{table*}







==> tables/results_1.tex <==


\begin{table*}[ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
    \hline
        setting & ~ & cs-en & de-en & et-en & fi-en & ru-en & tr-en & zh-en & avg \\ \hline
        m(y*,y) & BLEU & 23\% & 42\% & 29\% & 15\% & 23\% & 15\% & 18\% & 23\% \\ \hline
        ~ & YISI-1 & 32\% & 49\% & 35\% & 23\% & 30\% & 23\% & 21\% & 31\% \\ \hline
        m(x,y) & M-BERT & 1\% & 23\% & 18\% & 12\% & 10\% & 4\% & 8\% & 11\% \\ \hline
        ~ & LASER & 7\% & 32\% & 25\% & 16\% & 10\% & 9\% & 6\% & 15\% \\ \hline
        ~ & XMoverScore & 8\% & 28\% & 21\% & 15\% & 15\% & 9\% & 12\% & 15\% \\ \hline
        ~ & XMoverScore + LM & 29\% & 46\% & 23\% & 32\% & 26\% & 16\% & 19\% & 27\% \\ \hline
        ~ & TeacherSim & 13\% & 17\% & 17\% & 23\% & 26\% & 21\% & 15\% & 19\% \\ \hline
        ~ & TeacherSim + LM & 31\% & 45\% & 33\% & 24\% & 28\% & 22\% & 17\% & 29\% \\ \hline
    \end{tabular}
    \label{tab:wmt18-to-en}
\end{table*}


